Symbolic Register Automata for Complex Event Recognition and Forecasting

We propose an automaton model which is a combination of symbolic and register automata, i.e., we enrich symbolic automata with memory. We call such automata Symbolic Register Automata (SRA). SRA extend the expressive power of symbolic automata, by allowing Boolean formulas to be applied not only to the last element read from the input string, but to multiple elements, stored in their registers. SRA also extend register automata, by allowing arbitrary Boolean formulas, besides equality predicates. We study the closure properties of SRA under union, intersection, concatenation, Kleene closure, complement and determinization and show that SRA, contrary to symbolic automata, are not in general closed under complement and they are not determinizable. However, they are closed under these operations when a window operator, quintessential in Complex Event Recognition, is used. We show how SRA can be used in Complex Event Recognition in order to detect patterns upon streams of events, using our framework that provides declarative and compositional semantics, and that allows for a systematic treatment of such automata. We also show how the behavior of SRA, as they consume streams of events, can be given a probabilistic description with the help of prediction suffix trees. This allows us to go one step beyond Complex Event Recognition to Complex Event Forecasting, where, besides detecting complex patterns, we can also efficiently forecast their occurrence.

==> proofs_isomorphism.tex <==
\ifdefined\FI
\begin{lemma}
For every \dsra\ $A_{s}$ there exists a deterministic classical finite automaton  $A_{c}$ such that $\mathcal{L}(A_{c})$ is the set of strings induced by applying $N=\mathit{Minterms}(\mathit{Predicates}(A_{s}))$ to $\mathcal{L}(A_{s})$.
\end{lemma}
\else
\begin{lemma*}
For every \dsra\ $A_{s}$ there exists a deterministic classical finite automaton  $A_{c}$ such that $\mathcal{L}(A_{c})$ is the set of strings induced by applying $N=\mathit{Minterms}(\mathit{Predicates}(A_{s}))$ to $\mathcal{L}(A_{s})$.
\end{lemma*}
\fi

\begin{proof}
From an algebraic point of view,
the set $N=\mathit{Minterms}(\mathit{Predicates}(M))$ may be treated as a generator of the monoid $N^{*}$, 
with concatenation as the operation.
If the cardinality of $N$ is $k$,
then we can always find a set $\Sigma=\{a_{1},\cdots,a_{k}\}$ of $k$ distinct symbols and then a morphism (in fact, an isomorphism) $\phi: N^{*} \rightarrow \Sigma^{*}$ that maps each minterm to exactly one, unique $a_{i}$.
A classical automaton $A_{c}$ can then be constructed by relabeling the \dsra\ $A_{s}$ under $\phi$,
i.e.,
by copying/renaming the states and transitions of the original \dsra\ $A_{s}$ and by replacing the label of each transition of $A_{s}$ by the image of this label under $\phi$.
Then, the behavior of $A_{c}$ (the language it accepts) is the image under $\phi$ of the behavior of $M_{s}$ \cite{DBLP:books/daglib/0023547}.
Or, equivalently, the language of $A_{c}$ is the set of strings induced by applying $N=\mathit{Minterms}(\mathit{Predicates}(A_{s}))$ to $\mathcal{L}(A_{s})$.
\end{proof}
